Investigating the Impact of Interpersonal Challenges on Feeling Welcome in OSS

The sustainability of open source software (OSS) projects hinges on contributor retention. Interpersonal challenges can inhibit a feeling of welcomeness among contributors, particularly from underrepresented groups, which impacts their decision to continue with the project. How much this impact is, varies among individuals, underlining the importance of a thorough understanding of their effects. Here, we investigate the effects of interpersonal challenges on the sense of welcomeness among diverse populations within OSS, through the diversity lenses of gender, race, and (dis)ability. We analyzed the large-scale Linux Foundation Diversity and Inclusion survey (n = 706) to model a theoretical framework linking interpersonal challenges with the sense of welcomeness through Structural Equation Models Partial Least Squares (PLS-SEM). We then examine the model to identify the impact of these challenges on different demographics through Multi-Group Analysis (MGA). Finally, we conducted a regression analysis to investigate how differently people from different demographics experience different types of interpersonal challenges. Our findings confirm the negative association between interpersonal challenges and the feeling of welcomeness in OSS, with this relationship being more pronounced among gender minorities and people with disabilities. We found that different challenges have unique impacts on how people feel welcomed, with variations across gender, race, and disability groups. We also provide evidence that people from gender minorities and with disabilities are more likely to experience interpersonal challenges than their counterparts, especially when we analyze stalking, sexual harassment, and doxxing. Our insights benefit OSS communities, informing potential strategies to improve the landscape of interpersonal relationships, ultimately fostering more inclusive and welcoming communities.

==> IPMA-backup.tex <==
To answer RQ3, we employed Importance-Performance Map Analysis (IPMA) in PLS-SEM, which combines the analysis of the importance and performance dimensions of the PLS-SEM investigation~\cite{ringle2016gain} and has been used in the software engineering domain~\cite{russo2021agile}. IPMA enables researchers to gain richer and more precise insights from their findings because it simultaneously considers both the path coefficients' estimates and the average values of the latent variable scores. In our study, the PLS-SEM analysis performed for RQ1 and RQ2 allowed us to understand the magnitude of the effects of the independent variable, interpersonal challenges, on feeling welcome, the dependent variable.

However, this analysis did not evaluate the average values of the indicators that are part of the independent latent variable. In other words, it did not consider whether, according to participants’ ratings, feeling welcome performed worse in terms of each of the interpersonal challenges. The joint evaluation of these constructs’ importance (i.e., of their effects on feeling welcome) and performance (i.e., of their average values) enabled us to complement PLS-SEM results with relevant insights to guide managerial action. We investigate the extent to which the indicators from the construct \textit{Interpersonal Challenges} affect the target construct (\textit{Feeling Welcome}). 

Figure \ref{fig:IPMA-overall-population} represents the combination of the constructs’ importance and performance for the overall population. \textit{Doxxing} is the interpersonal challenge that presents the highest relative importance on not feeling welcome, followed by \textit{Sexual Harassment} and \textit{Stalking}.

\begin{figure}[!htb]
\centering
\includegraphics[width=3.5in]{Figures/IPMA-all.png}
\caption{Importance-Performance Map Analysis of Feeling Welcome for all respondents}
\label{fig:IPMA-overall-population}
\end{figure}


Understanding the distinctions of critical interpersonal challenges between demographic groups can inform targeted interventions to improve feelings of welcome within these groups. 

%As we did not find any differences between the association of interpersonal challenges and welcomeness for race, 

We investigated the interplay between the importance and performance of constructs for gender minorities (Fig. \ref{fig:IPMA-gender}.a) and men (Fig. \ref{fig:IPMA-gender}.b), between race minorities (Fig. \ref{fig:IPMA_race}.a) and white contributors (Fig. \ref{fig:IPMA_race}.b), and between contributors who live with disabilities (Fig. \ref{fig:IPMA_disabilities}.a) and contributors with no disabilities \ref{fig:IPMA_disabilities}.b).

Regarding gender, we observe a similar order of indicators as the most impactful on feeling welcome (as depicted in Fig. \ref{fig:IPMA-gender}. The most substantial reduction in feeling welcome is associated with the occurrence of \textit{Sexual Harassment}, followed by \textit{Doxxing} and \textit{Stalking}. Men showed almost a similar criticality of \textit{Sexual Harassment} and \textit{Doxxing}, while gender minorities had a higher prevalence of \textit{Sexual Harassment} when related to not feeling welcome than \textit{Doxxing}.

We observed that for Non-White individuals, \textit{Doxxing} emerges as the most critical indicator, while for White individuals, \textit{Lack of Response or Rejection of Contributions or Questions} takes precedence as the most crucial indicator.



\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/IPMA-gender.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges Associated with Feeling Welcome, per groups of gender} 
\label{fig:IPMA-gender}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/ipma-race.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated with Feelings Welcome, per groups of race} 
\label{fig:IPMA_race}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/ipma-disabilities.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated with Feelings Welcome, per disabilities} 
\label{fig:IPMA_disabilities}
\end{figure*}

%When examining IPMA between groups of individuals with disabilities (Fig.\ref{fig:IPMA_disabilities}.a) and with no disabilities (Fig.\ref{fig:IPMA_disabilities}.b), we observe that \textsc{Doxxing} is the most critical indicator for people who identify having disabilities. For people who identify as not having any kind of disability, \textsc{Sexual Harassment} is the most critical interpersonal challenge associated with them to feel welcome, yet very close to \textsc{Doxxing}.


%\begin{figure*}[htb]
%\centering
%\includegraphics[width=1\textwidth]{Figures/ipma-disabilities.png}
%\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated to Feeling Welcome, per having or not disabilities} 
%\label{fig:IPMA_disabilities}
%\end{figure*}

To enhance the sense of welcome for gender minorities, the community should prioritize strengthening measures against sexual harassment and doxxing. On the other hand, for men, White individuals, and those without disabilities, efforts should focus on issues related to unresponsiveness, rejection of contributions or questions, and general conflicts among contributors. Stereotyping and unwelcoming language, while still interpersonal challenges, exhibited a relatively weaker association with the feeling of being unwelcome compared to other challenges. More detailed results are discussed in the next section.


==> IPMAbackup.tex <==
To answer RQ3, we employed Importance-Performance Map Analysis (IPMA) in PLS-SEM, which combines the analysis of the importance and performance dimensions of the PLS-SEM investigation~\cite{ringle2016gain} and has been used in the software engineering domain~\cite{russo2021agile}. IPMA enables researchers to gain richer and more precise insights from their findings because it simultaneously considers both the path coefficients' estimates and the average values of the latent variable scores. In our study, the PLS-SEM analysis performed for RQ1 and RQ2 allowed us to understand the magnitude of the effects of the independent variable, interpersonal challenges, on feeling welcome, the dependent variable.

However, this analysis did not evaluate the average values of the indicators that are part of the independent latent variable. In other words, it did not consider whether, according to participants’ ratings, feeling welcome performed worse in terms of each of the interpersonal challenges. The joint evaluation of these constructs’ importance (i.e., of their effects on feeling welcome) and performance (i.e., of their average values) enabled us to complement PLS-SEM results with relevant insights to guide managerial action. We investigate the extent to which the indicators from the construct \textit{Interpersonal Challenges} affect the target construct (\textit{Feeling Welcome}). 

Figure \ref{fig:IPMA-overall-population} represents the combination of the constructs’ importance and performance for the overall population. \textit{Doxxing} is the interpersonal challenge that presents the highest relative importance on not feeling welcome, followed by \textit{Sexual Harassment} and \textit{Stalking}.

\begin{figure}[!htb]
\centering
\includegraphics[width=3.5in]{Figures/IPMA-all.png}
\caption{Importance-Performance Map Analysis of Feeling Welcome for all respondents}
\label{fig:IPMA-overall-population}
\end{figure}


Understanding the distinctions of critical interpersonal challenges between demographic groups can inform targeted interventions to improve feelings of welcome within these groups. 

%As we did not find any differences between the association of interpersonal challenges and welcomeness for race, 

We investigated the interplay between the importance and performance of constructs for gender minorities (Fig. \ref{fig:IPMA-gender}.a) and men (Fig. \ref{fig:IPMA-gender}.b), between race minorities (Fig. \ref{fig:IPMA_race}.a) and white contributors (Fig. \ref{fig:IPMA_race}.b), and between contributors who live with disabilities (Fig. \ref{fig:IPMA_disabilities}.a) and contributors with no disabilities \ref{fig:IPMA_disabilities}.b).

Regarding gender, we observe a similar order of indicators as the most impactful on feeling welcome (as depicted in Fig. \ref{fig:IPMA-gender}. The most substantial reduction in feeling welcome is associated with the occurrence of \textit{Sexual Harassment}, followed by \textit{Doxxing} and \textit{Stalking}. Men showed almost a similar criticality of \textit{Sexual Harassment} and \textit{Doxxing}, while gender minorities had a higher prevalence of \textit{Sexual Harassment} when related to not feeling welcome than \textit{Doxxing}.

We observed that for Non-White individuals, \textit{Doxxing} emerges as the most critical indicator, while for White individuals, \textit{Lack of Response or Rejection of Contributions or Questions} takes precedence as the most crucial indicator.



\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/IPMA-gender.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges Associated with Feeling Welcome, per groups of gender} 
\label{fig:IPMA-gender}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/ipma-race.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated with Feelings Welcome, per groups of race} 
\label{fig:IPMA_race}
\end{figure*}

\begin{figure*}[htb]
\centering
\includegraphics[width=1\textwidth]{Figures/ipma-disabilities.png}
\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated with Feelings Welcome, per disabilities} 
\label{fig:IPMA_disabilities}
\end{figure*}

%When examining IPMA between groups of individuals with disabilities (Fig.\ref{fig:IPMA_disabilities}.a) and with no disabilities (Fig.\ref{fig:IPMA_disabilities}.b), we observe that \textsc{Doxxing} is the most critical indicator for people who identify having disabilities. For people who identify as not having any kind of disability, \textsc{Sexual Harassment} is the most critical interpersonal challenge associated with them to feel welcome, yet very close to \textsc{Doxxing}.


%\begin{figure*}[htb]
%\centering
%\includegraphics[width=1\textwidth]{Figures/ipma-disabilities.png}
%\caption{Importance-Performance Map Analysis of Interpersonal Challenges associated to Feeling Welcome, per having or not disabilities} 
%\label{fig:IPMA_disabilities}
%\end{figure*}

To enhance the sense of welcome for gender minorities, the community should prioritize strengthening measures against sexual harassment and doxxing. On the other hand, for men, White individuals, and those without disabilities, efforts should focus on issues related to unresponsiveness, rejection of contributions or questions, and general conflicts among contributors. Stereotyping and unwelcoming language, while still interpersonal challenges, exhibited a relatively weaker association with the feeling of being unwelcome compared to other challenges. More detailed results are discussed in the next section.


==> OldIntro.tex <==
\begin{comment}
    
%--------------------------OLD-------------------------
%What is missing, however, is an understanding of how the challenges faced by individuals with different demographic attributes are knitted into their feeling of welcomeness in the community, which in turn creates an impassable barrier for diverse contributors to make sustained and meaningful contribution to OSS. While prior work investigated how intrinsic factors such as membership, identity, belonging, and attachment to a group result in a Sense of Virtual Community (SVC) in OSS \cite{trinkenreich2023belong}, it does not tie this feeling of SVC to the challenges that individuals face, which are the antecedents to SVC. This oversight is not trivial, the feeling of welcomeness is key to sustained engagement, particularly in environments built upon open collaboration principles~\cite{forte2013defining}.
%
%Previous research also investigated the Sense of Virtual Community in OSS \cite{trinkenreich2023belong}.% that includes membership, identity, belonging, and attachment to a group that primarily interacts through electronic communication. 
%
%The present study focuses on the \textbf{Feeling of Welcomeness}, which precedes belongingness and is induced by a perception that the individual presence brings joy or satisfaction in someone else \cite{hailey2022racialized}. 
%To the best of our knowledge, no prior investigation has explored the effect of interpersonal challenges on the feeling of welcomeness by different populations.
Without a theoretical framework that articulates the association of the effects of challenges on the feeling of welcomeness by different segments of populations, strategies to retain diverse contributors are doomed to fail.


%In this paper, we investigate the association between interpersonal challenges and the feeling of welcomeness in OSS communities. 

Our study closes this gap through a large-scale (n=707), mixed-methods investigation of Linux Foundation survey data ~\cite{dei_survey}. It is guided by the following research questions:\\

\newcommand{\rqone}[1]{How are interpersonal challenges associated with the feeling of welcomeness in OSS?}

\vspace{-10pt}
\noindent \hangindent1em 
\textit{\textbf{RQ1.} \rqone{}}
\noindent Previous research has found that interpersonal challenges are part of the issues that affect inclusiveness in OSS projects \cite{trinkenreich2022women,balali2018newcomers}, which may be a reason for contributors to disengage. But what is unclear is its extent and the severity of its impact. A large-scale statistical model paves the way for future research on interventions by providing comparisons, identification of patterns or trends. Moreover, a model allows us to determine and delineate the different types of interpersonal challenges, their extent, and impact on feeling welcome, particularly for those who are in gender, race, or disability minorities. 
To answer this RQ, we build a theoretical model using Partial-Least Squares Structural Equation Modeling (PLS-SEM).
%\noindent Previous research had qualitatively found that interpersonal challenges affect inclusiveness in OSS projects \cite{trinkenreich2022women,balali2018newcomers} and may be a reason for contributors to disengage, but to the best of our knowledge, no other study quantified the strength of this association with statistical generalization that paves the way for future research with comparisons, identification of patterns or trends. Moreover, through this quantitative study we were able to find the heterogeneity of interpersonal challenges impact on feeling welcome for those who are in gender, race, or disability minorities.
\\
%We use Structural Equation Models - Partial Least Squares to test a theoretical model with the association between interpersonal challenges and (not) feeling welcome.

%RQ2. How does the association between interpersonal challenges and feeling welcome differ per gender, race, and disabilities?
\newcommand{\rqtwo}[1]{How does the association between interpersonal challenges and feeling welcome differ for those who are in gender, race, or disability minorities?}

\vspace{-10pt}
\noindent \hangindent1em
\textit{\textbf{RQ2.} \rqtwo{}}
\noindent Prior work has shown that interpersonal challenges tend to have a more pronounced impact on demographics typically underrepresented in the tech industry \cite{lee2019floss,balali2018,trinkenreich2022women}, but the impact of interpersonal challenges on the welcomeness across minority groups have not yet been quantified. Our analysis helps quantify which of the challenges disproportioantely impact the demographics. Such quantification is desperately needed to help OSS communities prioritize which challenges they need to eradicate since OSS projects are severely resource-constrained and include a host of challenges. 
We investigate how the impact of the different challenges varies for groups of gender, race, and disabilities through Multi-Group Analysis (MGA) and Mixed Effects Logistic Regression. 

%Then, we aim to explore a finer grain, identifying, through regression analyses, which of the interpersonal challenges influences the feeling of (un)welcomeness for each demographic group (gender, race, and disabilities). Previous research has not yet quantified the different interpersonal challenges of welcomeness across marginalized demographic groups, which is an important step toward creating a more diverse ecosystem.

%We use Multi-Group Analysis to compare the model obtained for RQ1 through demographic groups of gender (men vs. gender minorities), race (white vs. race minorities), and disabilities (those who live or not with disabilities).

%\newcommand{\rqthree}[1]{How do each of the interpersonal challenges impact the feeling of welcomeness for each demographic group?}

%\noindent \hangindent1em
%\textit{\textbf{RQ3.} \rqthree{}}

%\noindent In this RQ, we aim to explore a finer grain, identifying how each of the interpersonal challenges analyzed impacts the feeling of welcomeness for each demographic group (gender, race, and disabilities). Previous research has not yet quantified the different interpersonal challenges of welcomeness across marginalized demographic groups, which is an important step toward creating a more diverse ecosystem. \\

%\newcommand{\rqthree}[1]{Why do OSS contributors (do not) feel welcome?}

%We employed qualitative analysis on the open question of reasons to (not) feel welcome and segmented analysis per demographic groups of gender, race, and disabilities.

%We answer these questions within the context of OSS using 2,350 responses to a survey conducted by the Linux Foundation~\cite{dei_survey}. To answer RQ1, we built a theoretical model using Partial-Least Squares Structural Equation Modeling (PLS-SEM). For RQ2, we investigated whether the importance of these factors varies for groups of gender, race, and disabilities through Multi-Group Analysis (MGA) and Mixed Effects Logistic Regression. 

\noindent \hangindent1em
\textit{\textbf{Mixed-Methods Composite Assessment.}}
%In delving into the dynamics of (un)welcomeness within OSS communities, we strive to deepen our comprehension of the multifaceted factors at play. 
Finally, we followed a concurrent embedded strategy \cite{creswell2017research} and used qualitative analysis of the open-ended survey responses about reasons to feel (or not feel) welcome to understand the participants' specific experiences that contributed to their feeling (or lack) of welcomeness in the community. This served as a form of data triangulation of our work. 

%unveil how interpersonal challenges explain (not) feeling welcomeness in OSS.
%By understanding the specific reasons respondents experience or lack a feeling of welcomeness, we seek to gain a broader perspective at a different level of analysis of the nuanced nature of \cite{creswell2017research} how interpersonal challenges impact feeling welcome. This entails an exploration of their role in shaping individuals' feelings of (un)welcomeness in OSS.


Our model empirically shows that experiencing interpersonal challenges is negatively associated with feeling welcome in OSS. Moreover, it highlights the nuanced nature of how different challenges impact different demographics differently. For example, in our data, interpersonal challenges had a strong association with not feeling welcome for gender minorities and people with disabilities, but not for race. Respondents from race minorities felt less welcome when experiencing unwelcoming language, but this challenge did not significantly impact feeling welcomed for gender minorities nor people with disabilities in our data. 
%Doxxing impacts feeling welcome only for gender minorities, not for race minorities nor people with disabilities. 
%Both minorities and majorities feel discriminated against, and 
Stereotyping had no significant effect on the feeling of welcomeness for gender, race, or people with disabilities. But challenges such as stalking, sexual harassment, and lack of response or rejection of contributions made the three investigated minority groups feel less welcome than their counterparts.

%When confronted with interpersonal challenges, gender minorities and people with disabilities report feeling less welcome than men and contributors without any disability who also experienced interpersonal challenges. Stereotyping was the only interpersonal challenge that exhibited no significant difference in its influence on the perceived welcomeness among the three groups of minorities and majorities. Our findings revealed that both minorities and majorities reported feeling discriminated against and expressed a desire for fewer stereotypes within the community.

By understanding how specific challenges impact diverse contributors' feelings of welcomeness, our study not only advances the academic literature on the field of behavioral software engineering, but also holds practical implications. The results are paramount to inform OSS communities on the specific aspects to focus to foster diversity in OSS, which in turn can result in innovation, and drive the sustainability of OSS projects.
Our contributions offer valuable insights that may go beyond OSS, informing broader efforts in the software industry on how to create inclusive and equitable spaces.


%Our paper makes a novel contribution to the general field of behavioral software engineering by evaluating how different interpersonal challenges differently affect feeling of welcomeness in OSS for those who are in gender, race, or disability minority. OSS communities can utilize our findings to prioritize the barriers they need to fix to improve the feeling of welcomeness and retain diverse contributors. 
\end{comment}

==> Tables/codes.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Reasons for not feeling welcome in OSS}
\vspace{-0.3cm}
\label{tab:codes}
\footnotesize
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|l|l|r|r}
\hline
\rowcolor{gray!35}\multicolumn{2}{c}{ } & & \multicolumn{1}{c}{\textbf{ Men}} & \multicolumn{1}{c}{\textbf{Gender Minorities}} \\
\rowcolor{gray!35}&\textbf{Category} & \textbf{Description}& \multicolumn{1}{c}{\textbf{(total: xx)}} & \multicolumn{1}{c}{\textbf{(total: yyy)}} \\\hline\hline


\multirow{4}{*}{Interpersonal}
& No allys against harassment  &  xxxxxx & xxx (x\%) & xxx (x\%)\\\cline{2-5}
& Gatekeeping &  xxxxxx & xxx (x\%) & xxx (x\%)\\\cline{2-5}
& Language issues &  xxxxxx & xxx (x\%) & xxx (x\%)\\\cline{2-5}
& Discrimination against minorities &  xxxxxx & xxx (x\%) & xxx (x\%)\\\cline{2-5}
& Discrimination against majorities &  xxxxxx & xxx (x\%) & xxx (x\%)\\\cline{2-5}

\\\hline\hline
 
 
\multirow{4}{*}{Quad2}
& Advancement           & P1, P10, P12, P16, P20, P21, P22, P23, P24 & 9 & 8 (4\%)\\\cline{2-5}
& Performance           & P4                                         & 1 & 0 (0\%) \\\cline{2-5}
& Factual Contribution  & P2, P6, P12, P14, P18, P19, P20, P21       & 8 & 74 (38\%)\\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region in Q2}& \textbf{15} & \textbf{81} (42\%)\\\hline\hline

\rowcolor{gray!40}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region in Intra-personal} &
  11 &
  49 (25\%) \\ \hline\hline

\multirow{3}{*}{Quad3}
& Self-Development  & P7, P16, P18, P19, P20, P21, P24 & 7  & 19 (8\%)\\\cline{2-5}
& Creativity        & P10                              & 1  & 2 (1\%) \\\cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region in Q3}& \textbf{8} & \textbf{21} (11\%)\\\hline\hline

 
\multirow{3}{*}{Quad4} 
& Satisfaction  & P1, P5, P10, P16, P21, P26 & 6  & 14 (7\%)\\ \cline{2-5}
& Security      & P19, P24              & 2  & 17 (7\%)\\ \cline{2-5}
\rowcolor{gray!10}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region in Q4}&  \textbf{7} & \textbf{30 (16\%)} \\ \hline\hline



%\rowcolor{gray!20}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Affect} &  25 & 49 (25\%) \\ \hline

%\rowcolor{gray!20}\multicolumn{1}{r}{~}& \multicolumn{2}{r|}{Participants who mentioned at least one Region from Achievement} &  17 & 95 (49\%) \\ \hline

\hline

\end{tabular}}

\resizebox{0.75\textwidth}{!}{%
\tiny
\begin{tabular}{r}
\textbf{Quad1}: Interpersonal x Affect; \textbf{Quad2}: Interpersonal x Achievement; \textbf{Quad3}: Intrapersonal x Achievement; \textbf{Quad4}: Intrapersonal x Affect\\
The total per quadrant is not the sum of the regions since the participants often provided an answer that was categorized into \textbf{more than one region}.
\end{tabular}
}
\vspace{-0.2cm}

\end{table*}

==> Tables/cross_loadings.tex <==
\begin{table*}[!h]
\footnotesize
\centering
\caption{Cross loadings of the retained indicators on the constructs}
\label{tab:cross_loadings}
\begin{tabular}{p{0.2cm}
                p{5.5cm}
                P{12mm}
                P{12mm}
                P{12mm}
                P{12mm}
                P{12mm}
                P{12mm}
                P{10mm}}
\toprule
& & {Leadership Support} & {Org. Culture} & {Opp. to Learn} & Engagement & Burnout & {Job Satisfaction} & {Intention to Stay}\\
\midrule
SL1 & Leaders encourage healthy balance between personal and professional activities & \textbf{.785} & .554 & .482 & .411 & -.543 & .436 & .359\\
SL2 & I would work with my leaders again & \textbf{.813} & .582 & .529 & .441 & -.461 & .474 & .414\\
SL3 & My leaders and I have meaningful conversations about my career interests and how to reach my career goals 
& \textbf{.742} & .512 & .528 & .370 & -.372 & .413 & .331\\
SL4 & My leaders care about my well-being 
& \textbf{.831} & .579 & .495 & .387 & -.448 & .455 & .377\\
SL5 & My leaders recognize and value my work 
& \textbf{.793} & .596 & .537 & .415 & -.416 & .441 & .380\\

\midrule
OC1 & Failures are seen as learning opportunities
&
.509 & \textbf{.689} & .493 & .396 & -.426 & .484 & .357\\
OC2 & I am empowered to make decisions needed to my job
&
.518 & \textbf{.729} & .489 & .467 & -.417 & .421 & .336\\
OC3 & I feel encouraged to come up with innovative and disruptive solutions
&
.511 & \textbf{.752} & .540 & .513 & -.487 & .481 & .399\\
OC4 & I feel safe speaking up and taking risks
&
.475 & \textbf{.710} & .432 & .406 & -.418 & .413 & .310\\
OC5 & Responsibilities are shared in my team
&
.532 & \textbf{.693} & .456 & .420 & -.439 & .408 & .327\\
OC6 & There is good teamwork and cooperation between different areas
&
.486 & \textbf{.679} & .510 & .424 & -.459 & .490 & .386\\
\midrule
OL1 & I am given different learning experiences to continue boosting my current skills and learning new ones
&
.483 & .524 & \textbf{.775} & .498 & -.446 & .456 & .391\\
OL2 & I believe I have enough opportunities to develop and grow my career
&
.551 & .581 & \textbf{.852} & .525 & -.517 & .609 & .548\\
OL3 & I feel my performance results and commitment contribute to my career development
&
.537 & .568 & \textbf{.805} & .500 & -.471 & .532 & .453\\
\midrule
EN1 & I am enthusiastic about my job
&
.488 & .552 & .590 & \textbf{.854} & -.566 & .559 & .501\\
EN2 & I wake up energized in the morning and am ready to begin a new work day
&
.398 & .495 & .485 & \textbf{.808} & -.644 & .499 & .418\\
EN3 &  Time flies when I'm working
&
.341 & .453 & .430 & \textbf{.766} & -.405 & .426 & .360\\
\midrule
BT1 & I'm becoming less interested in work
&
-.396 & -.437 & -.495 & .-603 & \textbf{.678} & -.488 & -.472\\
BT2 & I feel I can blend personal professional activities in healthy way (reversed)
&
-.498 & -.535 & -.476 & .-471 & \textbf{.794} & -.483 & -.386\\
BT3 & I feel mentally and physically exhausted from work
&
-.340 & -.359 & -.344 & .-434 & \textbf{.744} & -.357 & -.325\\
BT4 & I feel my current workload is manageable (reversed)
&
-.431 & -.462 & -.386 & .-375 & \textbf{.712} & -.378 & -.356\\
BT5 & I feel well physically, mentally and spiritually (reversed)
&
-.423 & -.488 & -.457 & .-579 & \textbf{.772} & -.448 & -.373\\
\midrule
JS1 & On a scale from 0 to 10, how likely are you to recommend TechCom as a workplace to your friends or former colleagues?
&
.513 & .557 & .573 & .521 & -.517 & \textbf{.867} & .598\\
JS2 & I feel proud to be part of TechCom
&
.472 & .546 & .582 & .560 & -.531 & \textbf{.896} & .620\\
JS3 & I feel that I belong to TechCom
&
.492 & .571 & .582 & .542 & -.504 & \textbf{.873} & .587\\

\midrule
IS1 & I rarely think about looking for a job at another company
&
.352 & .372 & .420 & .388 & -.387 & .466 & \textbf{.812}\\
IS2 & I see myself working at TechCom for the next year
&
.452 & .481 & .560 & .519 & -.502 & .690 & \textbf{.919}\\

\bottomrule

\end{tabular}
\end{table*}

==> Tables/internal_consistency.tex <==
\begin{table}[!hb]
\centering
\caption{Internal Consistency Reliability}
\vspace{-3mm}
\label{tab:internal_consistency_reliability}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,    
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=2, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{p{3.5cm}
                S[table-format=1.2]
                S[table-format=1.2]
                S[table-format=1.2]}
\toprule
& {\makecell{Cronbach's \textalpha}} & {\makecell{CR}} & {AVE}\\
\midrule
Leadership Support & .853 & .895 & .630\\
Organizational Culture & .802 & .858 & .503\\
Opportunities to Learn & .739 & .852 & .658\\
Engagement & .739 & .851 & .656\\
Burnout & .795 & .859 & .549\\
Job Enthusiasm & .853 & .911 & .772\\
Intention to Stay & .680 & .858 & .752\\
\bottomrule


\end{tabular}
\end{table}

==> Tables/mixed_effect.tex <==
\begin{table*}[htb]
\centering
%\scriptsize
\caption{Odds Ratios of feeling welcomed Based on Different Demographics}
\label{tab:mixed}
\resizebox{0.68\textwidth}{!}{
%\resizebox{\columnwidth}{!}{
\begin{tabular}{llllll}
\hline
\multicolumn{1}{c}{\textbf{Challenges}}                        & \textbf{Variance}                 & \textbf{AIC}                 & \multicolumn{1}{c}{\textbf{Race Minorities}}                 & \multicolumn{1}{c}{\textbf{Gender Minorities}}                & \multicolumn{1}{c}{\textbf{Disability}}                \\ \hline
Base model                                                     &                                   & 375.02                       & \textbf{0.53*}                                               & \textbf{0.28**}                                               & \textbf{0.44**}                                        \\
Lack of Response or Rejection of Contributions                 & 1.28                              & 343.00                       & \textbf{0.53*}                                               & \textbf{0.34**}                                               & \textbf{0.51*}                                         \\
Conflict with Other Contributors                               & 0.79                              & 351.65                       & \textbf{0.49*}                                               & \textbf{0.33**}                                               & 0.61                                                   \\
Unwelcoming Language                                           & 2.26                              & 304.70                       & \textbf{0.42**}                                              & 0.57                                                          & 0.73                                                   \\
Stalking                                                       & 1.21                              & 337.70                       & \textbf{0.54*}                                               & \textbf{0.41**}                                               & \textbf{0.52*}                                         \\
Sexual harassment                                              & 0.44                              & 365.78                       & \textbf{0.53*}                                               & \textbf{0.41**}                                               & \textbf{0.52*}                                         \\
Stereotyping                                                   & 2.36                              & 300.46                       & 0.59                                                         & 0.60                                                          & 0.63                                                   \\
Doxxing                                                        & 0.62                              & 355.55                       & 0.60                                                         & \textbf{0.31**}                                               & 0.57                                                   \\ \hline
\multicolumn{6}{l}{\begin{tabular}[c]{@{}l@{}}An odds ratio of less than 1 indicates that the minority group of each demographic feels less welcomed compared to \\ the majority group. A single asterisk (*) means p-value of coefficient \textless 0.05, and a double asterisk (**) means  \textless 0.01\end{tabular}}
\end{tabular}
}



\end{table*}

==> Tables/model_metrics.tex <==
\begin{table}[!hb]
\centering
\caption{Predictions Metrics from Algorithms}
\vspace{-3mm}
\label{tab:model_metrics}
\robustify{\bfseries}
\sisetup{
    mode=text,
    group-digits = false ,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,    
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places, 
    round-precision=3, %% change this for precision.
    parse-numbers = true
}
\begin{tabular}{p{2.7cm}
                S[table-format=0.3]
                S[table-format=0.3]
                S[table-format=0.3]}
\toprule
Algorithm & {Precision} & {Recall} & {F-Measure} \\ 
\midrule 
DecisionTree & \bfseries .979 & \bfseries .978  & \bfseries .978 \\
RandomForestClassifier & .978 & .977 & .977 \\
KNeighborsClassifier   & .930 & .929 & .929 \\
MLPClassifier          & .852 & .840 & .840 \\
Gaussian NB              & .518 & .519 & .518 \\
LogisticRegression     & .512 & .511 & .511 \\
LinearSVC               & .512 & .511 & .510 \\
DummyClassifier        & .499 & .500 & .500  \\  
\bottomrule
\end{tabular}

\end{table}

==> Tables/persisting_challenges.tex <==
\begin{table}[htb]
\centering
\caption{Which of the interpersonal challenges do you think still persist in 2024?}
\label{tab:persistent}
\resizebox{\columnwidth}{!}{
\footnotesize
\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}c  }
\hline
\multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{Challenges}} & \multicolumn{1}{c}{\cellcolor[HTML]{FFFFFF}\textbf{\% responses (n=30)}}  \\ \hline
Lack of Response or Rejection of Contributions                  & 47\% (17)                                                                 \\
Conflict with Other Contributors                                & 44\% (16)                                                        \\
Unwelcoming Language                                            & 28\% (10)                                                             \\
Stalking                                                        & 19\% (7)                                                              \\
Sexual harassment                                               & 28\% (10)                                                              \\
Stereotyping                                                    & 36\% (13)                                                             \\
Doxxing                                                         & 25\% (9)                                                              \\ \hline
\end{tabular}}
\resizebox{0.7\columnwidth}{!}{%
\begin{tabularx}{\columnwidth}{X}
%\begin{tabularx}{\linewidth}{@{}@{}}
The answer was optional, and respondents could consider more than one challenge persists, so the number of responses does not sum to 34 and percentages do not sum to 100\%\end{tabularx}
}

\end{table}

==> arxiv.tex <==
\input{Tables/logistic}


\textbf{Gender minorities and people with disabilities more frequently face interpersonal challenges in OSS.}


\boldification{Table shows the logistic regression analysis of the prevalence of interpersonal challenges that each demographic minority faces...}
%
Table~\ref{tab:logistic} shows the logistic regression analysis of the prevalence of interpersonal challenges that each demographic minority faces. The table highlights the odds ratio of variables that show statistical significance at $p$ < 0.05 or $p$ < 0.01, denoted by * or **, respectively. Odds ratios of less than 1.0 mean lower odds; odds ratios larger than 1.0 mean higher odds. For instance, in the model for \textsc{Lack of Response or Rejection of Contributions}, both gender minority and disability variables are statistically significant. The odds ratio for gender minorities is 1.56, indicating that \textsc{individuals identified as gender minorities are 1.56 times more likely than men to face this challenge compared to non-minorities.} Similarly, people with disabilities are 1.6748 significantly more likely to experience this challenge than those with no disabilities.


\boldification{all challenges are more likely faced by gender minorities than by men...}
%
As shown in Table~\ref{tab:logistic}, all challenges are more likely faced by gender minorities than by men, and all challenges (except doxxing) are more likely faced by people with disabilities than those who do not have any disability. 


\boldification{Our findings corroborate existing research, highlighting that gender minorities in OSS face significant socio-cultural challenges...}
%
\textit{Challenges experienced by gender minorities:} Our results confirm previous research \cite{trinkenreich2022women} that showed the socio-cultural challenges experienced by gender minorities when contributing to OSS, as \textsc{sexual harassment} (odds 14.75) \cite{calvo2020visible,singh2019women,nafus2012patches}, \textsc{stereotyping} (odds 4.11) \cite{powell2010gender}, \textsc{unwelcomming language} (odds 4.23) \cite{paul2019expressions,balali2018newcomers,qiu2019signals}, and \textsc{lack of response or rejection of contributions or questions} (1.56), and conflicts with other contributors (odds 1.92) \cite{vasilescu2015perceptions,nafus2012patches,imtiaz2019investigating}. \cite{canedo2020work,terrell2017gender,bosu2019diversity}. Regarding the two challenges not yet explored by OSS literature, we showed that have more odds to affect gender minorities than men: \textsc{stalking} (odds 7.13) and \textsc{doxxing} (odds 3.51).



\boldification{Our findings also highlight that disability more likely to face interpersonal challenges...}
%
Our analysis reveals that the most significant challenge people with disabilities often face is \textsc{unsolicited sexual advances or comments}, indicating that people with disabilities are more than three times as likely to encounter such challenges compared to contributors without disabilities. Equally concerning is the higher frequency of facing challenges including \textsc{conflict with other contributors}, \textsc{unwelcoming language}, and \textsc{unsolicited sexual advances or comments}, which reveals that people with disabilities are twice as likely to encounter these challenges compared to contributors without disabilities. The other two challenges that are statistically significant for models of \textsc{Lack of response or rejection of contributions} and \textsc{stereotyping based on perceived demographics} also disproportionately affect people with disabilities.


\MyBox{RQ3a. Gender minorities and individuals with disabilities are more likely to encounter interpersonal challenges; the highest odds ratio for gender minorities is for sexual harassment, and for people with disabilities, it is for stalking.}

==> formatting.tex <==
%%
%% Klaas's secret formatting code.
%%
\usepackage{bookmark}
\usepackage[authoryear]{natbib}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{microtype}
\usepackage{booktabs}
\usepackage[mode=text]{siunitx}
\usepackage{etoolbox}
\usepackage{enumitem} 
\usepackage{textgreek}
\usepackage{tipa}
\usepackage{url}
\usepackage{ragged2e}
\usepackage{caption}
\usepackage{times}



%\captionsetup[table]{font=footnotesize,labelfont={bf,sf},labelsep=quad,justification=RaggedRight,singlelinecheck=0}

\captionsetup[figure]{font=footnotesize,labelfont={sf,bf},labelsep=period,singlelinecheck=0,margin=0pt}



\widowpenalty10000
\clubpenalty10000

\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}p{#1}}
\usepackage{makecell}

\newcommand\hypothesis[2]{\vspace{0.5em} \noindent \hangindent=1em \textbf{Hypothesis #1 (H#1).} {#2}\vspace{0.5em}}



\usepackage[
paperwidth=15.51cm,
paperheight=23.52cm,
margin=0.65in
]{geometry}


\usepackage{hyperref}
\hypersetup{
 colorlinks=true,   
 citecolor=blue,
 urlcolor=blue,
 linkcolor=blue,
 bookmarksnumbered=true,     
 bookmarksopen=true,         
 bookmarksopenlevel=1,       
 colorlinks=true,            
 pdfstartview=Fit,           
 pdfpagemode=UseOutlines,    
 pdfpagelayout=TwoPageRight 
}

\usepackage{titlesec}

\usepackage[lining]{FiraSans} 
\usepackage[T1]{fontenc}

\titleformat{\section}
  {\sffamily\bfseries\fontsize{11}{13}\selectfont}{\thesection}{1em}{}

\titleformat{\subsection}
  {\sffamily\bfseries\fontsize{10}{12}\selectfont}{\thesubsection}{1em}{}

\titleformat{\subsubsection}
  {\sffamily\bfseries\itshape\fontsize{9}{11}\selectfont}{\thesubsubsection}{0.5em}{}



==> info.tex <==

References from ICSE 23:

Minimum sample size:

 For establishing an appropriate sample size, we conducted apriori power analysis using the G* power tool [90]. The maximum number of predictors in our model is 1 which indicates a minimum sample size of 54 and our sample of <> exceeded it considerably. 


 Barlett's and KMO:

 There are two recommended tests for ensuring the dataset's suitability for factor analysis [93, 94]. First, we conducted Bartlett's test of sphericity [93] on our constructs. The computed p-value (< 2.2e-16) is significant indicating that the factor analysis is useful. Next, we computed the Kaiser-Meyer-Olikn (KMO) measure of sampling adequacy. The result (0.87) was way above the recommended threshold (0.60) [94].

 

 

==> old_mixed.tex <==
%(i) In the first step, we built seven separate logistic regression models, with each interpersonal challenge as the dependent variable for each model. The independent binary variables are gender minorities, race minorities, and disabilities (Table \ref{tab:demographics}). This approach allows us to assess which demographic group will likely encounter specific interpersonal challenges. Since the dependent variable was categorical from a 4-point Likert-scale response (Never, rarely, occasionally, and frequently), we then grouped the response into binary variables to no (Never and rarely) and yes (occasionally and frequently). 


%(ii) With the understanding from step (i), we then 
% The dependent variable is from a 5-point Likert-scale response in agreement with the feeling of welcomeness. We followed previous research \cite{feng2023state1} and converted the responses of agreement in the feeling of being welcomed (5-point Likert-scale response) into a binary variable as the dependent variable. The ``Disagree" group combined ``Strongly disagree" and ``Somewhat disagree," indicating unwelcomeness. The ``Non-disagree" group consisted of ``Neither agree nor disagree," ``Somewhat agree," and ``Strongly agree."  The fixed independent binary variables are gender minorities, race minorities, and disabilities. We built seven models utilizing each interpersonal challenge serving as random effects separately for each model so that we could understand whether the challenge impacted the feeling of welcomeness of the specific demographic group. 


% As the first step of Mixed-Effect Logistic Regression, we assess whether including the random effect is reasonable and improves the model fitting. Therefore, we conducted the Akaike Information Criterion (AIC) \cite{akaike2011akaike} and likelihood ratio test to assess the model fitting by comparing each model (with the random effect) to the base model (without random effect). For models in which random effect improves the model fitting, we then assessed the significance of each independent variable (demographic groups) to understand the impact of the challenge on different groups feeling welcomed. 

% Both fixed and mixed-effect regressions were built with one model for each challenge. In the fixed-effect the challenge is the dependent variable. In the mixed-effect, the feeling welcomeness is the dependent variable and the challenge was treated as a random effect. 


%We grouped the gender and race demographics into dichotomic variables of gender minorities or only men and race minorities or only white, as presented in Table \ref{tab:demographics}. The disabilities are converted to binary variables as contributors with and without disabilities. 


% When comparing the fixed effects model with the model with random effects (on different challenges), we first examine the reduced Akaike Information Criterion (AIC). A decrease in AIC indicates that the inclusion of random effects not only improves the model fit but also justifies the added complexity. Additionally, we employ the chi-square test to assess the significance of including random effects. For instance, a low p-value signifies a statistically significant difference in fit between the two models, providing strong evidence to reject the null hypothesis in favor of the alternative: incorporating random effect parameters significantly enhances the model's explanatory power compared to the base model without random effects. Subsequently, by examining the model with random effects, we can identify which variables are statistically significant, shedding light on how specific interpersonal challenges (random effects) influence feeling welcome for different demographic contributors.


%Having or not having disabilities was already a dichotomic variable, and we did not do any transformation.
 
%This binary categorization simplifies the analysis while still capturing the essence of participants' feelings towards being welcomed.



% The seven models (one per each interpersonal challenge) were defined according to the formula below.

%Therefore, the dependent variable for all models was feeling welcome as a dichotomic variable, the fixed variables are demographic attributes, and the random variables represent each interpersonal challenge. We then compared the coefficient of the significant results to find the interpersonal challenges that acted as most impactful for each demographic group to feel welcome.

% $Y_i = \beta_0 + \beta_1 \cdot \text{Gender minotiry}_i + \beta_2 \cdot \text{Race minotiry}_i + \beta_3 \cdot \text{Disability}_i + \varepsilon_i,$

%To fit the logistic regression model, we reclassified the $Y_i$ into dichotomic for each model, representing ``Never'' and ``Rarely'' as (0) and ``Occasionally'' and ``Frequently'' as (1).

% The results from the logistic regression models showed the impact of demographic factors on the prevalence of interpersonal challenges. To investigate how these challenges affect the feeling of welcomeness for different demographic groups, we investigated whether individuals from various demographic backgrounds felt welcome and if different challenges influenced these feelings. 


% \begin{equation}
% \label{eq:base_model}
% feel welcome = \beta_0 + \beta_1X_1 + \beta_2X_2 + \cdots + \beta_nX_n
% \end{equation}
% \begin{equation}
% \label{eq:mixed_effect}
% feel welcome = \beta_0 + \beta_1X_1 + \beta_2X_2 + \cdots + \beta_nX_n + u_j
% \end{equation}\\



%Section~\ref{sec:results_measurement_model} presents the results of several procedures to evaluate the validity of the measurement model.

%After the quantitative analysis, we qualitatively analyzed the open question to understand the reasons why the contributors (do not) feel welcome in OSS.

==> oldmixed.tex <==
%(i) In the first step, we built seven separate logistic regression models, with each interpersonal challenge as the dependent variable for each model. The independent binary variables are gender minorities, race minorities, and disabilities (Table \ref{tab:demographics}). This approach allows us to assess which demographic group will likely encounter specific interpersonal challenges. Since the dependent variable was categorical from a 4-point Likert-scale response (Never, rarely, occasionally, and frequently), we then grouped the response into binary variables to no (Never and rarely) and yes (occasionally and frequently). 


%(ii) With the understanding from step (i), we then 
% The dependent variable is from a 5-point Likert-scale response in agreement with the feeling of welcomeness. We followed previous research \cite{feng2023state1} and converted the responses of agreement in the feeling of being welcomed (5-point Likert-scale response) into a binary variable as the dependent variable. The ``Disagree" group combined ``Strongly disagree" and ``Somewhat disagree," indicating unwelcomeness. The ``Non-disagree" group consisted of ``Neither agree nor disagree," ``Somewhat agree," and ``Strongly agree."  The fixed independent binary variables are gender minorities, race minorities, and disabilities. We built seven models utilizing each interpersonal challenge serving as random effects separately for each model so that we could understand whether the challenge impacted the feeling of welcomeness of the specific demographic group. 


% As the first step of Mixed-Effect Logistic Regression, we assess whether including the random effect is reasonable and improves the model fitting. Therefore, we conducted the Akaike Information Criterion (AIC) \cite{akaike2011akaike} and likelihood ratio test to assess the model fitting by comparing each model (with the random effect) to the base model (without random effect). For models in which random effect improves the model fitting, we then assessed the significance of each independent variable (demographic groups) to understand the impact of the challenge on different groups feeling welcomed. 

% Both fixed and mixed-effect regressions were built with one model for each challenge. In the fixed-effect the challenge is the dependent variable. In the mixed-effect, the feeling welcomeness is the dependent variable and the challenge was treated as a random effect. 


%We grouped the gender and race demographics into dichotomic variables of gender minorities or only men and race minorities or only white, as presented in Table \ref{tab:demographics}. The disabilities are converted to binary variables as contributors with and without disabilities. 


% When comparing the fixed effects model with the model with random effects (on different challenges), we first examine the reduced Akaike Information Criterion (AIC). A decrease in AIC indicates that the inclusion of random effects not only improves the model fit but also justifies the added complexity. Additionally, we employ the chi-square test to assess the significance of including random effects. For instance, a low p-value signifies a statistically significant difference in fit between the two models, providing strong evidence to reject the null hypothesis in favor of the alternative: incorporating random effect parameters significantly enhances the model's explanatory power compared to the base model without random effects. Subsequently, by examining the model with random effects, we can identify which variables are statistically significant, shedding light on how specific interpersonal challenges (random effects) influence feeling welcome for different demographic contributors.


%Having or not having disabilities was already a dichotomic variable, and we did not do any transformation.
 
%This binary categorization simplifies the analysis while still capturing the essence of participants' feelings towards being welcomed.



% The seven models (one per each interpersonal challenge) were defined according to the formula below.

%Therefore, the dependent variable for all models was feeling welcome as a dichotomic variable, the fixed variables are demographic attributes, and the random variables represent each interpersonal challenge. We then compared the coefficient of the significant results to find the interpersonal challenges that acted as most impactful for each demographic group to feel welcome.

% $Y_i = \beta_0 + \beta_1 \cdot \text{Gender minotiry}_i + \beta_2 \cdot \text{Race minotiry}_i + \beta_3 \cdot \text{Disability}_i + \varepsilon_i,$

%To fit the logistic regression model, we reclassified the $Y_i$ into dichotomic for each model, representing ``Never'' and ``Rarely'' as (0) and ``Occasionally'' and ``Frequently'' as (1).

% The results from the logistic regression models showed the impact of demographic factors on the prevalence of interpersonal challenges. To investigate how these challenges affect the feeling of welcomeness for different demographic groups, we investigated whether individuals from various demographic backgrounds felt welcome and if different challenges influenced these feelings. 


% \begin{equation}
% \label{eq:base_model}
% feel welcome = \beta_0 + \beta_1X_1 + \beta_2X_2 + \cdots + \beta_nX_n
% \end{equation}
% \begin{equation}
% \label{eq:mixed_effect}
% feel welcome = \beta_0 + \beta_1X_1 + \beta_2X_2 + \cdots + \beta_nX_n + u_j
% \end{equation}\\



%Section~\ref{sec:results_measurement_model} presents the results of several procedures to evaluate the validity of the measurement model.

%After the quantitative analysis, we qualitatively analyzed the open question to understand the reasons why the contributors (do not) feel welcome in OSS.
